Evading Classifiers by Morphing in the Dark

Learning-based systems have been shown to be vulnerable to evasion through adversarial data manipulation. These attacks have been studied under assumptions that the adversary has certain knowledge of either the target model internals, its training dataset or at least classification scores it assigns to input samples. In this paper, we investigate a much more constrained and realistic attack scenario wherein the target classifier is minimally exposed to the adversary, revealing on its final classification decision (e.g., reject or accept an input sample). Moreover, the adversary can only manipulate malicious samples using a blackbox morpher. That is, the adversary has to evade the target classifier by morphing malicious samples "in the dark". We present a scoring mechanism that can assign a real-value score which reflects evasion progress to each sample based on the limited information available. Leveraging on such scoring mechanism, we propose an evasion method -- EvadeHC -- and evaluate it against two PDF malware detectors, namely PDFRate and Hidost. The experimental evaluation demonstrates that the proposed evasion attacks are effective, attaining $100\%$ evasion rate on the evaluation dataset. Interestingly, EvadeHC outperforms the known classifier evasion technique that operates based on classification scores output by the classifiers. Although our evaluations are conducted on PDF malware classifier, the proposed approaches are domain-agnostic and is of wider application to other learning-based systems.

==> approach.tex <==
\section{Evading Binary Classifiers}
In this section, we describe two generic techniques to evade learning-classifiers. Both of our techniques start with a malicious variant which is correctly classified by the target classifier, and then modify or ``mutate" it to derive an evasive variant which possesses the same malicious functionality as the original one does, but misclassified as benign by the target classifier. Prior to describing the two techniques, we first define a mutator function $\cal M$ which mutates malicious variants during the course of the evasion. 

\subsection{Mutator}
While the adversary $\cal A$ can manipulate a malicious sample in various ways, without loss of generality, we can model the manipulation by a mutator $\cal M$. $\cal M$ is a function that takes as input a sample $x$, a random seed $r$, and a numerical parameter $d \in [0,1]$, and outputs $x' \gets {\cal M}(x, r,d)$. The random seed $r$ is used to decide what modification to be made on $x$, while the numerical parameter $d$ decides level of the modification. For example, if $x$ is a PDF file comprising of a set of objects, $d$ indicates how many objects of $x$ is to be modified (with $d=0$ means modification while $d=1$ means all objects in $x$ are to be modified) and $r$ decides what action to be made on the objects (e.g., insert, replace or delete). 


\subsection{Binary Search}

\subsection{Hill Climbing}
%\input{figures/PDFRate_score_change}
%\input{figures/PDFRate_b2b_change}

%\input{figures/Hidost_score_change}
%\input{figures/Hidost_b2b_change}

==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

In this section, we first give a brief background on machine learning classifiers and then discuss recent studies which show these classifiers are likely susceptible to malicious data manipulation.

\subsection{Machine Learning Classifiers}
Machine learning is a generic method which attempts to ``learn" from existing data (or training data) to gain an ability to make predictions on future data (or operational data). Machine learning classifiers are a particular kind of learning systems that classifies new data into two or more predefined classes. For example, a PDF malware classifier, on input of a PDF file $x$, would predict if $x$ is benign or malicious. 

Without loss of generality, a classifier can be represented by a tuple $\langle f, T \rangle$ where in $f$ is an unique mechanism by which the classifier evaluates an input data point $x$ and derives some probabilistic score $f(x)$, and $T$ is a threshold (or a set of thresholds) against which the derived probabilistic scores $f(x)$ are compared. The result of such comparison decides the output of the classifier on an input $x$. 

There are various techniques to ``learn" $\langle f, T \rangle$ from a given training dataset~\cite{SVM,grad_des}. While differ in their mechanisms, they share a common purpose of configuring $f$ and $T$ such that the error rate on the training dataset is minimal. Such configuration results in high accuracy when operating on operational data if the training data and the operational data have the same distribution. 

When being deployed in security tasks, machine learning systems do not execute and examine behaviour of suspicious samples in real system, but rather rely on their static properties to predict their maliciousness. Although many systems have reported impressive results~\cite{ML_high_accuracy, hidost}, it remains a question whether the static properties that they consider are fundamentally essential to the malicious behaviours, or they are merely superficial artefacts that both training and operational data happen to have in common. If it is the latter case, these systems are likely vulnerable to malicious data manipulation. 

\subsection{Evading Machine Learning Classifiers}
When critical decision making which has non-trivial economic or security implications is outsourced to a machine-learning system, there certainly exist various incentives for the adversaries to maliciously influence its decision so as to gain unfair advantage. Examples of systems which are potentially subject to such attacks are spam detection~\cite{evade_spam_detection}, adversarial advertisements~\cite{evade_adv_ad}, automatic signature generator~\cite{evade_worm_sign}.

For security tasks that employ a machine-learning classifier, the adversary's object is often to confuse the classifier so that it labels a malicious instance as benign. Intuitively, detailed knowledge of the classifier significantly benefits the adversary in conducting evasion attacks. {\v{S}}rndic et al.~\cite{evade_adhoc_14} proposed a taxonomy of evasion scenarios based on the knowledge about the target classifier's components that are available to the adversary. These components include {\em training datasets} and {\em classification algorithms} together with their parameters, as well as a {\em feature set} that the classifier has learnt. The authors report successful evasion attacks for different scenarios wherein the adversary has high level of knowledge about the target system's feature set. Xu et al.~\cite{evademl} consider a stronger adversary that does not has any internal information about the classifier, assuming black-box access to the target system and relying on classification scores that it assigns to submitted variants to stage the evasion attacks. The authors, nevertheless, acknowledge that their attacks are rendered infeasible if the assumed auxiliary information are hidden. 





